How to deal with malleability of BitCoin transactions

BitCoin transactions are malleable in a sense that given a transaction an adversary can easily construct an equivalent transaction which has a different hash. This can pose a serious problem in some BitCoin distributed contracts in which changing a transaction's hash may result in the protocol disruption and a financial loss. The problem mostly concerns protocols, which use a "refund" transaction to withdraw a deposit in a case of the protocol interruption. In this short note, we show a general technique for creating malleability-resilient "refund" transactions, which does not require any modification of the BitCoin protocol. Applying our technique to our previous paper "Fair Two-Party Computations via the BitCoin Deposits" (Cryptology ePrint Archive, 2013) allows to achieve fairness in any Two-Party Computation using the BitCoin protocol in its current version.

==> new-notbot-graph.tex <==
% !TEX root = malleability.tex

\trans{-3, 0}{5.0}
  {t}{$\CS.\Commit(\inp~T)$}
  {$\sig_{B}(\BODY{\CS.\Commit})$}
  {$body, \sigma_1, \sigma_2, x$}
  {\\ $(\ver_{B}(body, \sigma_1) \land H(x) = h_B) \;\lor$ \\
    $(\ver_{B}(body, \sigma_1) \land \ver_{A}(body, \sigma_2))$}
  {$d\,\BTC$};
    
\trans{1, -3}{3.4}
  {td}{$\CS.\Open(\inp~\CS.\Commit)$}
  {$\sig_{B}(\BODY{\CS.\Open}), \bot, s_B$}
  {$body, \sigma$}
  {$\ver_{B}(body, \sigma)$}
  {$d\,\BTC$};

\Dtrans[$t$]{-5.5, -3}{5.}
  {tr}{$\CS.\Fuse(\inp~\CS.\Commit)$}
  {\\ $\sig_{B}(\BODY{\CS.\Fuse}), \sig_{A}(\BODY{\CS.\Fuse}), \bot$}
  {$body, \sigma$}
  {$\ver_{A}(body, \sigma)$}
  {$d\,\BTC$};

\draw [->] ([xshift=1.5cm]t.south) |- 
  (td.west)
  node[midway, xshift=0.3cm, yshift=0.7cm]{$d\,\BTC$};

\draw[dotted] [->] ([xshift=0.8cm]t.south) |- 
  (tr.east)
  node[midway, xshift=-0.3cm, yshift=0.7cm]{$d\,\BTC$};

\draw [<-] (t.east) -- ++(0.8,0)
  node[midway, yshift=0.2cm]{$d\,\BTC$};
  
\draw [->] (td.east) -- ++(0.8,0)
  node[midway, yshift=0.2cm]{$d\,\BTC$};
  
\draw[dotted] [->] (tr.west) -- ++(-0.8,0)
  node[midway, yshift=0.2cm]{$d\,\BTC$};

\trans{-2.5,-6.}{4.3}
    {t0}{$\PutMoney(\inp~T^\sA)$}
    {$\sig_{\sA}(\BODY{\PutMoney})$}
    {$\body,\sigma,x$}
    {$\ver_{A}(\body,\sigma) \land H(x) = h_B$}
    {$d\,\BTC$};

%\trans{0,-6}{5}
%    {t1}{$\FuseNB(\inp~\PutMoney)$}
%    {$\sig_{C}(\BODY{\FuseNB}), r_S$}
%    {$\body,\sigma$}
%    {$\ver_{C}(\body,\sigma)$}
%    {$d\,\BTC$};


\draw [<-] ([yshift=0.3cm] t0.west) -- ++(-0.8,0cm)
  node[midway, xshift=0.0cm, yshift=0.2cm]{$d\,\BTC$};
  
\draw [->] ([yshift=-0.3cm] t0.west) -- ++(-0.8,0cm)
  node[midway, xshift=0.0cm, yshift=0.2cm]{$d\,\BTC$};  


%\draw [->] (t0.east) -- (t1.west)
  %node[midway, xshift=0cm, yshift=0.20cm]{$d\,\BTC$};


%\draw [->] (t1.south) |- (-0.80,-7.5)
  %node[midway, xshift=-0.4cm, yshift=0.2cm]{$d\,\BTC$};


==> trick-desc.tex <==
\begin{enumerate}
\item[]
    \begin{center} {\bf Pre-conditions:} \end{center} 
\vspace{0.1cm}
  \item $\sA$ holds the key pair $A$ and $\sB$ holds the key pair $B$.
\end{enumerate}
\begin{enumerate}
\item[]
    \begin{center} {\bf The commitment phase:} \end{center}
\vspace{0.1cm}
  \item The parties execute the $\ARCom(\sB, \sA, d, t, r)$ protocol.
  \item $\sA$ creates the $\PutMoney$ transaction using the value $h$ from the transaction $\AR(\sB, \sA, d, t, r).\Commit$ and broadcasts it.
    \begin{center} {\bf The opening phase:} \end{center}
\vspace{-0.2cm}
  \item $\sB$ opens the commitment revealing $r$ just before time $t$.
  \item $\sA$ broadcasts the $\Fuse$ transaction at time $t$ (if $\PutMoney$ was not spent earlier).
  \item If $\sB$ has not opened the commitment until time $t$, then $\sA$ gains $d\,\BTC$
  from the $\AR(\sB, \sA, d, t, r).\Fuse$ transaction.
\end{enumerate}

